An exponentially convergent discretization for space-time fractional parabolic equations using $hp$-FEM

We consider a space-time fractional parabolic problem. Combining a sinc-quadrature based method for discretizing the Riesz-Dunford integral with $hp$-FEM in space yields an exponentially convergent scheme for the initial boundary value problem with homogeneous right-hand side. For the inhomogeneous problem, an $hp$-quadrature scheme is implemented. We rigorously prove exponential convergence with focus on small times $t$, proving robustness with respect to startup singularities due to data incompatibilities.

==> figures/contour.tex <==
\begin{tikzpicture}[scale=0.7]
\fill[fill=blue!10] (-1.2,-4) -- (2,-4) -- (2,4) -- (-1.2,4) -- cycle ;
\fill[fill=blue!10] let \p1= (22.5:7) in 
(2,0) -- (22.5:7) -- (\x1,4) -- (2,4) ;

\fill[fill=blue!10] let \p1= (-22.5:7) in
(2,0) -- (-22.5:7) -- (\x1,-4) -- (2,-4) ;


\draw[dashed,fill=white] (0,0) circle (0.5);
\node (eps) at (-0.8,0.2) {$\varepsilon_0$};

\draw[<->] (-1.5,0) -- (6.5,0);
\draw[<->] (0,-4.5) -- (0,4.5);

%\draw[thick] (0,0) -- (45:5);
%\draw[color=white] (0,0) -- (45:1);

%\draw[thick] (0,0) -- (-45:5);
%\draw[color=white] (0,0) -- (-45:1);

\node (c) at (2.2,2.5) {$\mathcal{C}$};
%\node (c2) at (1.25,0.24) {$\mathcal{C}_2$};
%\node (c3) at (1,1.5) {$\mathcal{C}_3$};
%\node[font=\huge] (s) at (4,2.5) {$ \mathcal{S}$};



%\draw[thick] (0,0) ++(-45:1)  arc (-45:45:1) ;

\draw[thick, domain=-3:3, samples=15,smooth] plot ( {0.5*(2^\x+2^-\x)}, {0.5*(2^\x - 2^-\x)} ); 



\draw[dashed] (2,0) -- (22.5:7);
\draw[dashed] (2,0) -- (-22.5:7);
\node (z0) at (2,-0.3) {$z_0$};
\draw[fill,thick] (2,-0.1) -- (2,0.1);


\end{tikzpicture}

==> figures/l2error_sing.tex <==
\pgfplotsset{
  log x ticks with fixed point/.style={
      xticklabel={
        \pgfkeys{/pgf/fpu=true}
        \pgfmathparse{exp(\tick)}%
        \pgfmathprintnumber[fixed relative, precision=3]{\pgfmathresult}
        \pgfkeys{/pgf/fpu=false}
      }
  },
  log y ticks with fixed point/.style={
      yticklabel={
        \pgfkeys{/pgf/fpu=true}
        \pgfmathparse{exp(\tick)}%
        \pgfmathprintnumber[fixed relative, precision=3]{\pgfmathresult}
        \pgfkeys{/pgf/fpu=false}
      }
  }
}


\begin{tikzpicture}
  \begin{semilogyaxis}[
    width=\textwidth, height=6cm,     % size of the image
    %title=Condition Numbers,
    grid = major,
    grid style={dashed, gray!30},
    axis background/.style={fill=white},
    xlabel=$\Ndof^{1/4}$ ,
    ylabel= {Error},
    legend style={legend pos=south west, legend cell align=left,font=\small},
    %legend style={at={(0,-0.3)},anchor=north west,legend cell align=left},
    %xtick={1,10,100,1000},
    %xtick=
    %x tick label style={yshift=-0.5em,log x ticks with fixed point},
    %xmax=20000
    %log basis x = {10},
    %xtickten = { -2,-6,-10,-14},
    %xmax=0.1
    xmin=1
    ]
      
    % import the correct data from a CSV file
    % condition of not preconditioned
    \addplot+[solid,mark=square,mark size=1.5pt,mark options={line width=1.0pt},smooth,thick] table    
    [
    x expr= \thisrow{ndof}^(1/4),
    y=et1,
    col sep=space 
    ]{figures/data/error_sing.csv};    


    \addplot+[solid,mark=x,mark size=2pt,mark options={line width=1.0pt},smooth,thick] table    
    [
    x expr= \thisrow{ndof}^(1/4),
    y=et2,
    col sep=space 
    ]{figures/data/error_sing.csv};    

    \addplot+[solid,mark=o,mark size=1.5pt,mark options={line width=1.0pt},smooth,thick] table    
    [    
    x expr= \thisrow{ndof}^(1/4),
    y=et3,
    col sep=space 
    ]{figures/data/error_sing.csv};    

    
    
    \addplot [black,dashed ] expression [domain=6:20, samples=15] { 10*1*exp(-0.7*x)} node [pos=0.64,inner sep=2pt, anchor=south west] { $\bigO(e^{-0.7\,\Ndof^{\frac{1}{4}}})$};

    %\addplot [black,dashed ] expression [domain=6:50, samples=15] { 0.1*1*exp(-1*x)} node [pos=0.6,inner sep=2pt, anchor=south west] {$\small \bigO(e^{-2\,\Ndof^{1/4}})$};
    %\addplot [black,dashed ] expression [domain=0.01:1e-14, samples=15] { 1e-7*x^-(sqrt(2)/2)} node [pos=0.7,inner sep=2pt, anchor=south west] {$\bigO(t^{-\gamma})$};
    

    \legend{$t=0.001$, $t=0.1$, $t=1$};
  \end{semilogyaxis}
  \end{tikzpicture}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../sinc_parbolic_frac"
%%% End:


==> figures/l2error_smooth.tex <==
\pgfplotsset{
  log x ticks with fixed point/.style={
      xticklabel={
        \pgfkeys{/pgf/fpu=true}
        \pgfmathparse{exp(\tick)}%
        \pgfmathprintnumber[fixed relative, precision=3]{\pgfmathresult}
        \pgfkeys{/pgf/fpu=false}
      }
  },
  log y ticks with fixed point/.style={
      yticklabel={
        \pgfkeys{/pgf/fpu=true}
        \pgfmathparse{exp(\tick)}%
        \pgfmathprintnumber[fixed relative, precision=3]{\pgfmathresult}
        \pgfkeys{/pgf/fpu=false}
      }
  }
}


\begin{tikzpicture}
  \begin{semilogyaxis}[
    width=\textwidth, height=6cm,     % size of the image
    %title=Condition Numbers,
    grid = major,
    grid style={dashed, gray!30},
    axis background/.style={fill=white},
    xlabel=$\Ndof^{1/4}$ ,
    ylabel= {Error},
    legend style={legend pos=south west, legend cell align=left,font=\small},
    %legend style={at={(0,-0.3)},anchor=north west,legend cell align=left},
    %xtick={1,10,100,1000},
    %xtick=
    %x tick label style={yshift=-0.5em,log x ticks with fixed point},
    %xmax=20000
    %log basis x = {10},
    %xtickten = { -2,-6,-10,-14},
    %xmax=0.1
    xmin=1
    ]
      
    % import the correct data from a CSV file
    % condition of not preconditioned
    \addplot+[solid,mark=square,mark size=1pt,mark options={line width=1.0pt},smooth,thick] table    
    [
    x expr=\thisrow{ndof}^(1/4),%\thisrow{ndof}^(1/3),
    y = l2error,
    col sep=space
    ]{figures/data/error_smooth.csv};    

    
    
      \addplot [black,dashed ] expression [domain=4:20, samples=15] { 100*exp(-x)} node [pos=0.7,inner sep=2pt, anchor=south west] {$\bigO(e^{-\Ndof^{\frac{1}{4}}})$};
  
%    \addplot [black,dashed ] expression [domain=10:60, samples=15] { 10*2^(-x/2)} node [pos=0.8,inner sep=2pt, anchor=south west] {$\bigO(})$};
    %\addplot [black,dashed ] expression [domain=0.01:1e-14, samples=15] { 1e-7*x^-(sqrt(2)/2)} node [pos=0.7,inner sep=2pt, anchor=south west] {$\bigO(t^{-\gamma})$};
    

    \legend{$L^2$-error at $t=1$};
  \end{semilogyaxis}
  \end{tikzpicture}
%
%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../sinc_parbolic_frac"
%%% End:
%


==> figures/time_behavior_h1.tex <==
\pgfplotsset{
  log x ticks with fixed point/.style={
      xticklabel={
        \pgfkeys{/pgf/fpu=true}
        \pgfmathparse{exp(\tick)}%
        \pgfmathprintnumber[fixed relative, precision=3]{\pgfmathresult}
        \pgfkeys{/pgf/fpu=false}
      }
  },
  log y ticks with fixed point/.style={
      yticklabel={
        \pgfkeys{/pgf/fpu=true}
        \pgfmathparse{exp(\tick)}%
        \pgfmathprintnumber[fixed relative, precision=3]{\pgfmathresult}
        \pgfkeys{/pgf/fpu=false}
      }
  }
}


\begin{tikzpicture}
  \begin{loglogaxis}[
    width=0.6\textwidth, height=7cm,     % size of the image
    %title=Condition Numbers,
    grid = major,
    grid style={dashed, gray!30},
    axis background/.style={fill=white},
    xlabel=$t$ ,
    ylabel= {Error},
    legend style={legend pos=south west, legend cell align=left},
    %legend style={at={(0,-0.3)},anchor=north west,legend cell align=left},
    %xtick={1,10,100,1000},
    %xtick=
    %x tick label style={yshift=-0.5em,log x ticks with fixed point},
    %xmax=20000
    log basis x = {10},
    xtickten = { -2,-6,-10,-14},
    xmax=0.1
    ]
      
    % import the correct data from a CSV file
    % condition of not preconditioned
    \addplot+[solid,mark=square,mark size=1pt,mark options={line width=1.0pt},smooth,thick] table    
    [
    x=time,
    y=energy,
    col sep=space
    ]{figures/data/error_small_times2.csv};    

    \addplot+[solid,mark=square,mark size=1pt,mark options={line width=1.0pt},thick,smooth] table    
    [
    x=time,
    y=ltwo,
    col sep=space
    ]{figures/data/error_small_times2.csv};    

    
    
    \addplot [black,dashed ] expression [domain=0.01:1e-14, samples=15] { 8e-7*x^-(sqrt(2)/4)} node [pos=0.97,inner sep=2pt, anchor=south] {$\bigO(t^{-\gamma/2})$};
    \addplot [black,dashed ] expression [domain=0.01:1e-14, samples=15] { 1e-7*x^-(sqrt(2)/2)} node [pos=0.7,inner sep=2pt, anchor=south west] {$\bigO(t^{-\gamma})$};
    

    \legend{$H^1$-error,$L^2$-error};
  \end{loglogaxis} 
\end{tikzpicture}
%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../sinc_parabolic_frac"
%%% End:

